Meta-Learning Sparse Implicit Neural Representations

Implicit neural representations are a promising new avenue of representing general signals by learning a continuous function that, parameterized as a neural network, maps the domain of a signal to its codomain; the mapping from spatial coordinates of an image to its pixel values, for example. Being capable of conveying fine details in a high dimensional signal, unboundedly of its domain, implicit neural representations ensure many advantages over conventional discrete representations. However, the current approach is difficult to scale for a large number of signals or a data set, since learning a neural representation -- which is parameter heavy by itself -- for each signal individually requires a lot of memory and computations. To address this issue, we propose to leverage a meta-learning approach in combination with network compression under a sparsity constraint, such that it renders a well-initialized sparse parameterization that evolves quickly to represent a set of unseen signals in the subsequent training. We empirically demonstrate that meta-learned sparse neural representations achieve a much smaller loss than dense meta-learned models with the same number of parameters, when trained to fit each signal using the same number of optimization steps.

==> figs/computations.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{c c c }
        \toprule
        approach & computations (number of parameter update) & memory (of learnt INRs) \\
        \midrule
        baseline & $\mathcal{O}(Ndt)$ & $\mathcal{O}(Nd)$ \\
        compressing INRs & $\mathcal{O}(N (d t_{\text{pretrain}} + (\frac{\kappa + d}{2}) t_{\text{compress}} ) )$ & $\mathcal{O}(N \kappa)$ \\
        meta learning sparse INRs & ? & $\mathcal{O}(N \kappa)$ \\
        \bottomrule
    \end{tabular}
    \caption{\NL{1. Decide whether or not to put a table like this, 2. Update the table where possible/necessary; potentially this table can evolve to deliver more contents, 3. Not sure if this is the best place to put; maybe in a result section.}}
    \label{tab:complexities}
\end{table}

==> figs/lottery.tex <==
\begin{figure*}[t]
\centering
\subfigure[SIREN]{
\centering
\includegraphics[width=0.482\textwidth]{pngs/lottery/siren30.png}
}
\subfigure[Random Fourier Features]{
\centering
\includegraphics[width=0.482\textwidth]{pngs/lottery/ffn20.png}
}
\caption{
Comparisons of size-PSNR tradeoff curves for fitting a $512\times512$ image using dense and narrow models (red circles) and wide-sparse models pruned at initialization (blue squares).
Sparse models are pruned with iterative magnitude pruning with rewinding, that are known to yield ``winning ticket'' models.
In both plots, wide-sparse models do not perform noticeably well against narrow-dense models.
\textbf{Left:} MLP with sinusoidal activation functions.
\textbf{Right:} ReLU MLP with random Fourier feature encoding.
\NL{Perhaps mention what this result imply with regard to the main idea of this work.}
} 
 \label{fig:lottery}
\end{figure*}

==> figs/mainexp.tex <==
\begin{figure*}[t]
\centering
\subfigure[CIFAR-10]{
\centering
\includegraphics[width=0.482\textwidth]{pngs/main/cifar10.png}
}
\subfigure[CelebA]{
\centering
\includegraphics[width=0.482\textwidth]{pngs/main/celeba.png}
}
\subfigure[Imagenette]{
\centering
\includegraphics[width=0.482\textwidth]{pngs/main/imagenette.png}
}
\subfigure[SDF]{
\centering
\includegraphics[width=0.482\textwidth]{pngs/main/sdf.png}
}
\caption{
{\color{blue}Main plots; These will be updated with a three-seed version.}
\NL{weights -> parameters (for consistency)}
}
 \label{fig:main}
\end{figure*}

==> figs/schematics.tex <==
\begin{figure*}[t]
\centering
\subfigure[INR]{
\centering
\includegraphics[height=0.13\textheight]{pngs/schematics/upper_left.png}
}
\subfigure[Pruning INR for a single image using a standard pruning procedure \cite{han15}]{
\centering
\includegraphics[height=0.13\textheight]{pngs/schematics/upper_right.png}
}
\subfigure[The proposed SparseINR procedure for learning a sparse INR that can be trained further to fit each signal.]{
\centering
\includegraphics[height=0.13\textheight]{pngs/schematics/lower.png}
}

\caption{
Comparison of compression pipelines. \textbf{Left:} Standard pruning setup, where one iteratively trains and prunes the model fitted to a single target data. \textbf{Right:} Setup of this paper, where one iteratively meta-trains and prunes to generate a sparse, trainable representation that can be fine-tuned for each target data.
\NL{explain why single data (at least in the main text)}
}
 \label{fig:schematic}
\end{figure*}

==> texts/checklist.tex <==
\section*{Checklist}

\begin{enumerate}
\item For all authors...

\begin{enumerate}
\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \answerYes{}

\item Did you describe the limitations of your work? \answerYes{See \cref{sec:discussion}.}

\item Did you discuss any potential negative societal impacts of your work? \answerYes{See \cref{sec:discussion}.}

\item Have you read the ethics review guidelines and ensured that your paper conforms to them? \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
\item Did you state the full set of assumptions of all theoretical results? \answerNA{}
\item Did you include complete proofs of all theoretical results? \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \answerYes{See the supplemental materials.}
\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? \answerYes{See the supplemental material.}
\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
\answerYes{See \cref{ssec:mainexp}.}
\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
\answerYes{See the supplemental material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We use publicly available datasets, and have cited the reference.}
  \item Did you mention the license of the assets?
    \answerYes{See the supplemental material.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See the supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We use only publicly available datasets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? \answerYes{See the provided code.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable? \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable? \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? \answerNA{}
\end{enumerate}

\end{enumerate}
